Solving a real-world modular logistic scheduling problem with a quantum-classical metaheuristics

This study evaluates the performance of a quantum-classical metaheuristic and a traditional classical mathematical programming solver, applied to two mathematical optimization models for an industry-relevant scheduling problem with autonomous guided vehicles (AGVs). The two models are: (1) a time-indexed mixed-integer linear program, and (2) a novel binary optimization problem with linear and quadratic constraints and a linear objective. Our experiments indicate that optimization methods are very susceptible to modeling techniques and different solvers require dedicated methods. We show in this work that quantum-classical metaheuristics can benefit from a new way of modeling mathematical optimization problems. Additionally, we present a detailed performance comparison of the two solution methods for each optimization model.

==> sections/3_0_table.tex <==
\noindent

\begin{table*}[]
\centering

\tiny
\begin{tabular}{c|c|c|c|c|c|c|c} \hline\hline
 \multirow{2}{*}{\textbf{Id}} & \multirow{2}{*}{\textbf{A-Jobs}} & \multirow{2}{*}{\textbf{B-Jobs}} & \multirow{2}{*}{\textbf{$|T|$}} & \multirow{2}{*}{\textbf{$|K|$}} & \textbf{processing times} & \textbf{processing times} & \textbf{Runtime} \\ 
& & & & & \textbf{A-jobs} & \textbf{B-jobs} &\textbf{seconds} \\ \hline 
 1 & 3 & 3 & 215 & 2 & (5,4) & (4,5,4) & 5.08 \\ \hline
 2 & 4 & 4 & 60 & 3 & (5,3) & (2,3,2) & 5.25 \\ \hline
 3 & 3 & 3 & 64 & 4 & (6,5) & (5,6,5) & 5.28 \\ \hline
 4 & 3 & 3 & 125 & 2 & (7,6) & (4,6,4) & 5.56 \\ \hline
 5 & 3 & 3 & 129 & 2 & (6,5) & (5,6,5) & 5.85 \\ \hline
 6 & 4 & 4 & 40 & 5 & (3,2) & (2,3,2) & 5.95 \\ \hline
 7 & 4 & 4 & 42 & 5 & (4,3) & (3,4,3) & 6.17  \\ \hline
 8 & 4 & 4 & 52 & 4 & (4,3) & (3,4,3) & 6.36  \\ \hline
 9 & 3 & 3 & 60 & 5 & (7,6) & (6,7,6) & 6.43  \\ \hline
10 & 3 & 3 & 138 & 2 & (7,6) & (5,6,5) & 6.46  \\ \hline
11 & 3 & 3 & 259 & 1 & (6,5) & (5,6,5) & 6.71  \\ \hline
12 & 4 & 4 & 193 & 1 & (4,2) & (3,5,3) & 6.79  \\ \hline
13 & 4 & 4 & 105 & 2 & (4,3) & (3,4,3) & 6.94  \\ \hline
15 & 5 & 5 & 36 & 5 & (3,2) & (2,3,2) & 7.25  \\ \hline
16 & 3 & 3 & 277 & 1 & (7,6) & (5,6,5) & 7.43  \\ \hline
17 & 4 & 4 & 77 & 3 & (5,4) & (3,4,3) & 7.62  \\ \hline
18 & 4 & 4 & 211 & 1 & (4,3) & (3,4,3) & 7.73  \\ \hline
19 & 5 & 5 & 60 & 3 & (3,2) & (2,3,2) & 7.88  \\ \hline
20 & 4 & 4 & 116 & 2 & (5,4) & (3,4,3) & 7.96  \\ \hline
21 & 5 & 5 & 90 & 2 & (3,2) & (2,3,2) & 8.18  \\ \hline
22 & 4 & 4 & 53 & 5 & (5,4) & (4,5,4) & 8.82  \\ \hline
23 & 5 & 5 & 180 & 1 & (4,3) & (2,3,2) & 8.91  \\ \hline
24 & 4 & 4 & 127 & 2 & (6,5) & (3,5,3) & 9.0  \\ \hline
25 & 3 & 3 & 75 & 5 & (9,7) & (8,10,8) & 9.02  \\ \hline
26 & 5 & 5 & 184 & 1 & (4,2) & (2,4,2) & 9.12  \\ \hline
27 & 4 & 4 & 67 & 4 & (5,4) & (4,5,4) & 9.27  \\ \hline
28 & 4 & 4 & 89 & 3 & (5,4) & (4,5,4) & 9.44  \\ \hline
29 & 4 & 4 & 134 & 2 & (5,4) & (4,5,4) & 9.79  \\ \hline
30 & 5 & 5 & 105 & 2 & (5,3) & (2,3,2) & 9.9  \\ \hline
31 & 4 & 4 & 73 & 4 & (7,5) & (4,6,4) & 10.26  \\ \hline
32 & 4 & 4 & 268 & 1 & (5,4) & (4,5,4) & 10.9  \\ \hline
33 & 5 & 5 & 62 & 4 & (4,3) & (3,4,3) & 12.08  \\ \hline
34 & 4 & 4 & 65 & 5 & (6,5) & (5,6,5) & 12.15  \\ \hline
35 & 4 & 4 & 81 & 4 & (6,5) & (5,6,5) & 12.37  \\ \hline
36 & 4 & 4 & 294 & 1 & (7,5) & (4,5,4) & 12.44  \\ \hline
37 & 6 & 6 & 51 & 4 & (3,2) & (2,3,2) & 12.48  \\ \hline
38 & 4 & 4 & 108 & 3 & (6,5) & (5,6,5) & 12.57  \\ \hline
39 & 5 & 5 & 125 & 2 & (4,3) & (3,4,3) & 12.79  \\ \hline
40 & 6 & 6 & 68 & 3 & (3,2) & (2,3,2) & 12.82  \\ \hline
41 & 4 & 4 & 162 & 2 & (6,5) & (5,6,5) & 12.91  \\ \hline
42 & 6 & 6 & 103 & 2 & (3,2) & (2,3,2) & 13.37  \\ \hline
43 & 6 & 6 & 206 & 1 & (4,3) & (2,4,2) & 14.43  \\ \hline
44 & 6 & 6 & 206 & 1 & (4,3) & (2,3,2) & 14.44  \\ \hline
45 & 4 & 4 & 325 & 1 & (6,5) & (5,6,5) & 14.51  \\ \hline
46 & 4 & 4 & 182 & 2 & (7,5) & (6,7,6) & 15.29  \\ \hline
47 & 5 & 5 & 64 & 5 & (5,4) & (4,5,4) & 17.39  \\ \hline
48 & 5 & 5 & 80 & 4 & (5,4) & (4,5,4) & 17.63  \\ \hline
49 & 5 & 5 & 107 & 3 & (5,4) & (4,5,4) & 17.86  \\ \hline
50 & 4 & 4 & 382 & 1 & (7,6) & (6,7,6) & 18.57  \\ \hline
51 & 7 & 7 & 59 & 4 & (4,2) & (2,3,2) & 19.37  \\ \hline
52 & 7 & 7 & 58 & 4 & (3,2) & (2,3,2) & 19.58  \\ \hline
53 & 4 & 4 & 88 & 5 & (8,7) & (7,9,7) & 19.61  \\ \hline
54 & 5 & 5 & 321 & 1 & (5,4) & (4,5,4) & 20.02  \\ \hline
55 & 5 & 5 & 173 & 2 & (6,5) & (4,5,4) & 20.2  \\ \hline
56 & 6 & 6 & 58 & 5 & (4,3) & (3,4,3) & 20.43  \\ \hline
57 & 6 & 6 & 72 & 4 & (4,3) & (3,4,3) & 20.51  \\ \hline
58 & 6 & 6 & 96 & 3 & (4,3) & (3,4,3) & 20.7  \\ \hline
59 & 6 & 6 & 145 & 2 & (4,3) & (3,4,3) & 21.25  \\ \hline
60 & 7 & 7 & 233 & 1 & (4,3) & (2,3,2) & 22.03  \\ \hline
61 & 6 & 6 & 290 & 1 & (4,3) & (3,4,3) & 23.09  \\ \hline
62 & 5 & 5 & 195 & 2 & (6,5) & (5,6,5) & 24.15  \\ \hline
63 & 6 & 6 & 160 & 2 & (5,4) & (3,4,3) & 24.26  \\ \hline
64 & 5 & 5 & 84 & 5 & (8,6) & (5,6,5) & 25.82  \\ \hline
65 & 5 & 5 & 83 & 5 & (7,6) & (5,6,5) & 25.85  \\ \hline
66 & 5 & 5 & 104 & 4 & (7,6) & (5,6,5) & 26.09  \\ \hline
67 & 8 & 8 & 64 & 4 & (3,2) & (2,3,2) & 28.35  \\ \hline \hline
\end{tabular}
\caption{Problem instances used for benchmarking. The runtime is the by D-Wave computed instance specific runtime. The instances are ordered by runtime, which can be seen as a proxy for the instance size and hence the instance complexity. A solution to instance $28$ is visualized in Figure \ref{fig_problem}. The $k$-th  entry of the processing times tuple corresponds to the processing time of the $k$-th task.}
\label{table0}
\end{table*}
